MegaMath: Pushing the Limits of Open Math Corpora

Mathematical reasoning is a cornerstone of human intelligence and a key benchmark for advanced capabilities in large language models (LLMs). However, the research community still lacks an open, large-scale, high-quality corpus tailored to the demands of math-centric LLM pre-training. We present MegaMath, an open dataset curated from diverse, math-focused sources through following practices: (1) Revisiting web data: We re-extracted mathematical documents from Common Crawl with math-oriented HTML optimizations, fasttext-based filtering and deduplication, all for acquiring higher-quality data on the Internet. (2) Recalling Math-related code data: We identified high quality math-related code from large code training corpus, Stack-V2, further enhancing data diversity. (3) Exploring Synthetic data: We synthesized QA-style text, math-related code, and interleaved text-code blocks from web data or code data. By integrating these strategies and validating their effectiveness through extensive ablations, MegaMath delivers 371B tokens with the largest quantity and top quality among existing open math pre-training datasets.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/inst_model_math_cot_results.tex <==
\begin{table}[htbp]
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccccc}
    \toprule
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\diagbox{Model}{Benchmark}}} & \multicolumn{8}{c}{EN}\\
\cmidrule{2-9} & GSM8K & MATH  & \makecell{Minerva\\Math} & \makecell{GaoKao\\2023 En} & \makecell{Olympiad\\Bench} & \makecell{College\\Math} & \makecell{MMLU\\STEM} & \makecell{Avg.} \\
\midrule
    \multicolumn{9}{c}{\textbf{\textsc{Chain-of-Thought}}} \\ 
    \midrule
        GPT-4o-2024-08-06 & 92.9  & 81.1  & 36.8  & 67.5  & 43.3  & 48.5  & 64.2 & 62.0\\
    \midrule
    DeepSeekMath-7B-RL & 88.2  & 52.4  & 20.6  & 43.6  & 19.0  & 37.5  & 64.8 & 46.6  \\
    DeepSeek-Coder-V2-Lite-Instruct & 87.6  & 61.0  & 29.4  & 56.1  & 26.4  & 39.8  & 68.6 & 52.7   \\
    \midrule
    Internlm2-math-plus-7B & 84.0  & 54.4  & 17.3  & 50.1  & 18.8  & 36.2  & 55.2 & 45.1  \\
    Internlm2-math-plus-20B & 87.9  & 56.5  & 20.2  & 51.9  & 23.1  & 37.5  & 63.5 & 48.7 \\
    Internlm2-math-plus-mixtral8x7B & 92.1  & 59.4  & 26.8  & 49.6  & 25.0  & 37.5  & 71.9 & 51.8  \\
    \midrule
    Mathstral-7B-v0.1 & 84.9  & 56.6  & 16.2  & 46.0  & 21.5  & 33.7  & 64.0 & 46.1  \\
    \midrule
    NuminaMath-7B-CoT & 75.4  & 55.2  & 19.1  & 47.5  & 19.9  & 36.9  & 60.8 & 45.0   \\
    NuminaMath-72B-CoT & 90.8  & 66.7  & 25.0  & 58.4  & 32.6  & 39.7  & 64.5  & 54.0  \\
    \midrule
    Llama-3.1-8B-Instruct & 76.6  & 47.2  & 21.7  & 38.4  & 15.4  & 33.8  & 60.5 & 41.9    \\
    Llama-3.1-70B-Instruct & 94.1  & 65.7  & 34.2  & 54.0  & 27.7  & 42.5  & 80.4 & 56.9 \\
    \midrule
    Qwen2-1.5B-Instruct & 64.1  & 25.1  & 5.5   & 19.7  & 4.1   & 10.4  & 46.2  & 25.0 \\
    Qwen2-7B-Instruct & 85.7  & 52.9  & 19.5  & 36.4  & 21.3  & 24.5  & 68.2 & 44.1  \\
    Qwen2-72B-Instruct & 93.2  & 69.0  & 31.6  & 58.7  & 33.2  & 43.2  & \textbf{84.4} & 59.0  \\
    \midrule
    \multirow{2}[2]{*}{Qwen2-Math-1.5B-Instruct} & 84.2  & 69.4  & 29.4  & 59.7  & 31.3  & 44.2  & 54.9 & 53.3 \\
  & \hspace{0.63cm}88.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}75.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}32.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}63.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}37.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}46.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}59.5\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}57.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$} 
  \\
        & \hspace{0.5cm}92.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}79.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}36.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}68.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}43.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}46.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}74.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}63.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  \\
    \midrule
    \multirow{2}[2]{*}{Qwen2-Math-7B-Instruct} & 89.9  & 75.1  & 34.6  & 62.1  & 38.2  & 45.9  & 63.8 & 58.5   \\
      & \hspace{0.63cm}93.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}80.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}37.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}68.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}43.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}47.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}73.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}63.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}   \\

        & \hspace{0.5cm}95.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}83.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}39.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}71.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}47.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}47.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}78.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}66.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}   \\
    \midrule
    \multirow{2}[2]{*}{Qwen2-Math-72B-Instruct} & \textbf{96.7}  & 84.0  & 40.1  & 68.3  & 43.0  & 47.9  & 79.9 & 65.7  \\
          & \hspace{0.63cm}97.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}86.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}45.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}71.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}48.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}48.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}83.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}68.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  \\

        & \hspace{0.5cm}96.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}86.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}47.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}72.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}52.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}48.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}82.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}69.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-1.5B-Instruct}} & 84.8  & 75.8  & 29.4  &  65.5 & 38.1  & 47.7  &  57.5 & 56.9  \\
  & \hspace{0.63cm}89.5\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}80.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}32.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}68.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}43.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}48.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}60.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}60.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  \\
        & \hspace{0.5cm}94.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}83.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}37.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}73.0\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}47.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}50.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}65.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}64.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}   \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-7B-Instruct}} &  95.2 & 83.6  & 37.1  & 66.8  &  41.6 & 46.8 & 71.9 & 62.9 \\
      & \hspace{0.63cm}96.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}87.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}41.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}72.5\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}44.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}47.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}73.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}66.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}   \\

        & \hspace{0.5cm}97.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}88.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}42.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}75.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}49.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}49.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}78.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}68.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-72B-Instruct}} & 95.9  & \textbf{85.9}  & \textbf{44.1}  & \textbf{71.9}  & \textbf{49.0}  & \textbf{49.5}  &  80.8 & \textbf{68.2}  \\
          & \hspace{0.63cm}96.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}88.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}47.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}73.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}50.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}50.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}84.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}
          & \hspace{0.63cm}70.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}
          \\

        & \hspace{0.5cm}96.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}89.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}47.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}76.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}54.5\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} & \hspace{0.5cm}50.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} & \hspace{0.5cm}80.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} & \hspace{0.5cm}70.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}\\
         \midrule 
            \multicolumn{9}{c}{\textbf{\textsc{Tool-integrated Reasoning}}}
    \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-1.5B-Instruct}} & 83.7 & 79.9 & 33.5 & 67.8 & 49.2 & 54.8 & 56.9 & 60.8   \\
  & \hspace{0.63cm}90.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}85.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}35.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}71.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}54.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}56.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}60.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}64.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}    \\
        & \hspace{0.5cm}93.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}88.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}39.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}78.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}59.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}58.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}76.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}70.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-7B-Instruct}} & 94.6 & 85.2 & 39.0 & 71.4 & 55.6 & 56.0 & 70.1 & 67.4   \\
      & \hspace{0.63cm}96.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}89.9\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}40.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}76.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}58.6\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}57.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}71.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}70.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  \\

        & \hspace{0.5cm}97.6\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}91.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}42.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}80.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}63.1\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}58.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}82.2\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}73.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$} \\
    \midrule
    \multirow{2}[2]{*}{\textbf{Qwen2.5-Math-72B-Instruct}} & \textbf{95.8} & \textbf{88.1} & \textbf{48.2} & \textbf{75.3} & \textbf{60.6} & \textbf{57.7} & \textbf{82.3} & \textbf{72.6}  \\
          & \hspace{0.63cm}96.7\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}91.8\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}48.2\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}83.1\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}64.5\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}58.3\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}  & \hspace{0.63cm}85.0\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$}
          & \hspace{0.63cm}75.4\textcolor[RGB]{10, 0, 15}{$_{\texttt{maj@8}}$} \\

        & \hspace{0.5cm}96.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}92.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}49.3\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}83.4\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}65.9\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}59.7\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}90.0\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  & \hspace{0.5cm}76.8\textcolor[RGB]{84, 89, 247}{$_{\texttt{rm@8}}$}  \\
    \bottomrule
    \end{tabular}%
    }
     \caption{The results of Qwen2.5-Math-Instruct and other instruct models on English benchmarks. For CoT, we report few-shot pass@1 performance on MMLU(STEM) and zero-shot pass@1 performance on other benchmarks. For PoT, all benchmarks are evaluated in the zero-shot setting. Except for the pass@1 scores, we also provide the Qwen2-Math and Qwen2.5-Math performance with majority voting and reward model best-of-N among 8 sampled responses. Best pass@1 performance in CoT and TIR are marked in \textbf{bold}.}
\label{instruct_en_main_results}%

\end{table}%


